Ontology-Based Feedback to Improve Runtime Control for Multi-Agent Manufacturing Systems

Improving the overall equipment effectiveness (OEE) of machines on the shop floor is crucial to ensure the productivity and efficiency of manufacturing systems. To achieve the goal of increased OEE, there is a need to develop flexible runtime control strategies for the system. Decentralized strategies, such as multi-agent systems, have proven effective in improving system flexibility. However, runtime multi-agent control of complex manufacturing systems can be challenging as the agents require extensive communication and computational efforts to coordinate agent activities. One way to improve communication speed and cooperation capabilities between system agents is by providing a common language between these agents to represent knowledge about system behavior. The integration of ontology into multi-agent systems in manufacturing provides agents with the capability to continuously update and refine their knowledge in a global context. This paper contributes to the design of an ontology for multi-agent systems in manufacturing, introducing an extendable knowledge base and a methodology for continuously updating the production data by agents during runtime. To demonstrate the effectiveness of the proposed framework, a case study is conducted in a simulated environment, which shows improvements in OEE during runtime.

==> 30_framework_edit.tex <==
% What are the assumptions in designing an ontology
\subsection{Assumptions}
\label{subsec:assumptions}

In this paper, we make a number of assumptions. 
% assumption 1 (ontology with owl)
First, we assumed that an ontology is formalized using \gls{owl} for the framework in this paper. One of the strategies for creating a \gls{kb} in the field of \gls{mas} using \gls{swt} is developing the \gls{kb} in the form of an ontology. This approach allows for easy expansion of the \gls{kb} with new domain data and meeting specific requirements. Specifically, \gls{owl}[ 2 DL] is considered the best option for formalization, due to its high expressiveness and general decidability, 
making an ontology an ideal type of \gls{kb}. Furthermore, utilizing \gls{swt} allows for full utilization of the querying capabilities of the ontology. 
% assumption 2 (ontology with TBox and ABox)
The ontology is further put into a TBox (Terminological Box) and ABox (Assertional Box) structure. The TBox, which describes the concepts and relationships in the domain, is used to represent the classes and properties of the manufacturing system, such as products, resources, features, and processes. The ABox, on the other hand, is utilized for all instances (objects) of the concepts defined in the TBox and their relations. 
% assumption 3 (mas has pa and ra)
Additionally, an ontology is developed based on the architecture of a \gls{mas} that includes both \gls{pa} and \gls{ra}. The ontology will be designed to represent the knowledge about the production process, the resources, and the interactions between them. This will provide a common understanding and representation of the knowledge required for the MAS to operate effectively. 


% Assumptions -> Agents update ontology during runtime / have the capabilities to do so

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%       DESIGN OF THE FRAMEWORK       %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Design of the Framework}
\label{subsec:designOntology}

\begin{figure*}[t]
    \centering
    \includegraphics[width=.98\textwidth]{figures/figure-1-graphical-abstract.png}
    \caption{Graphical Abstract of the Framework}
    \label{fig:graphAbstract}
\end{figure*}

%Previous work done by Felix summarized in this paragraph roughly.
The framework presented in \Cref{fig:graphAbstract} provides an overall structure for the development of an ontology-enhanced multi-agent framework for runtime control of manufacturing systems. 
% Requirement 1 (extendable kb)
The framework utilizes an ontology as a centralized \gls{kb} to accumulate the state and production history of the \gls{mas}. This accumulated knowledge can be utilized to provide holistic environment models to the agents, providing a clear understanding of the current state and production history of the system. The agents are then able to make their respective decentralized decisions on a global context.
% Requirement 2 (plug and produce)
On one hand, engineers can construct an ontology by utilizing an ontology editor via spreadsheets, enabling "plug-and-produce" capabilities for flexibility and scalability. These spreadsheets provide the knowledge of product features, restrictions, and resource capabilities by being parsed into the \gls{kb}. 
% Requirement 3 (runtime control)
In addition to "plug-and-produce" capabilities, the framework provides capabilities for communication and coordination between agents and the ontology during the runtime of the manufacturing process. The agents can directly query and update the ontology through an \gls{api} interface during runtime, allowing for dynamic adjustments to the manufacturing process in response to global changes in resources, product features, or other factors. The encapsulation of the ontology inside an \gls{api} should further provide a lower barriers for agents to report their status updates.
% Interaction of Onotology providet holistic environment models and agent based decision making

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%       THE BASIC ONTOLOGY       %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subsection{The Basic Ontology}
\label{subsec:basicOntology}

\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figures/figure-2-base-tbox.png}
    \caption{Overview of the Ontology}
    \label{fig:baseTbox}
\end{figure}

The core concepts in the manufacturing system that is defined in the ontology include classes such as \textit{feature}, \textit{process}, \textit{resource}, and \textit{specification}. This is based on the \gls{ppr} model, in which \textit{resources} run \textit{processes} on \textit{products} to implement \textit{features} \cite{Nielsen2003}. 
% specification class
The \textit{specification} class refers to a detailed description of the desired product, including the specific features and requirements, as well as the expected deadline, as specified by the customer.
% process class
The \textit{process} class contains information on the production processes, which is a set of operations and procedures that transforms inputs info finished products including the use of resources such as robots and machines.
% resource class
The \textit{resource} class encompasses physical assets or capabilities that are used in the production process, including resources such as robots and buffers.
% features class
The \textit{feature} refers to the various characteristics or aspects of a product that are defined in a customer order and used to unambiguously describe the desired product with the process types.
% figurea
The initial TBox of ontology that includes this information is shown in \Cref{fig:baseTbox}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%       DEFINING THE RELATIONSHIPS       %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Defining the Relationship using Ontology}
\label{subsec:definingRelations}

\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figures/figure-3-relations-abox.png}
    \caption{Relationship among Products, Processes, Features and Resources}
    \label{fig:relationsAbox}
\end{figure}

To ensure that the \gls{mas} has the necessary information to make informed decisions about the production process and make any necessary modifications to achieve the desired outcomes, further relationships need to be defined for the classes of manufacturing systems. The central relationships are shown in \Cref{fig:relationsAbox}.

Three basic object properties are used for the main classes of manufacturing systems. First, resources are \textit{CapableOf} executing specific processes. Second, the process \textit{realizes} a feature. Third, the product \textit{defines} certain features. These basic properties define the main relationship among products, processes, features, and resources.

As the \gls{kb} should not only be able to represent the static \gls{mas}, but the dynamically changing environment including its events and actors further classes and properties have to be defined. 
In order to reflect the general desires of the agents in accordance to the BDI-architecture a linear objective function for a set of use-case specific metrics is proposed. This is represented in the ontology by the PA specific class \textit{objectiveFunction}. The link between objective function and the PA is created by the \textit{hasObjectiveFunction} property. The \textit{objectiveFunction} then has several \textit{coefficients} linked to it by the \textit{hasCoefficient} property. The value of the coefficient is is given by the \textit{hasValue} and the type of metric by the \textit{coefficientFor} datatype properties. To allow for an evaulation of processes, their respective performance also needs to be evaluated. This is done by introducing a \textit{performance} class and the \textit{hasPerformance} property. The \textit{hasPerformance} property has two subclasses, \textit{realPerformance} and \textit{expectedPerformance} to further enable transparency when it comes to historic decision making.
% hasPerformanceMetric instead of datatype properties
As a last metric each product also receives a \textit{deadline}.
Using the before-mentioned classes both the believes (by  environment models and expected performances) and desires (objective function and deadline) of the BDI-architecture can be represented.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%      Modeling the system during runtime      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Modeling the system during runtime}
\label{subsec:runtimeControl}

\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figures/figure-4-runtime-control.png}
    \caption{Example of a process execution in the Ontology}
    \label{fig:processExecution}
\end{figure}
While most of the \gls{mas} can be depicted using the up until now introduced ontology, neither the history or the plans of agents are currently added to the ontology. To support the inclusion of runtime data the \textit{processExecution} class is introduced. The previously introduced \textit{process} is a formal definition of actions to be performed by a resource to reach an outcome. A \textit{processExecution} however represents an instance of a \textit{process} being proposed, planned, executed or completed. A \textit{processExecution} therefore correlates to a physical event, while a \textit{process} represents the necessary actions to perform said event.

An example for a \textit{processExecution} is shown in \Cref{fig:processExecution}. A \gls{pa} adds each \textit{processExecution} to the ontology and displays its intention and actions in a globally accessible format. To connect each process execution to different parts of the base ontology, a new set of object properties is introduced. The \textit{hasProcessExecution} property associates a product with execution, while the \textit{runsOnResource} property indicates which resource is being utilized for the execution. Finally, the \textit{runsProcess} property links the underlying process to the execution and is added to the ontology.

The \textit{hasStatus} property is a crucial datatype property for the execution. It captures the different stages of the execution by assigning a literal value. Initially, the PA proposes the execution in the ontology by creating a \textit{processExecution} which \textit{hasStatus} "proposed". If both \gls{pa} and \gls{ra} agree and schedule the execution the status changes to "planned." When the execution starts, the status changes to "running" and then to "successful" if completed successfully. If unexpected events occur and the execution does not finish as planned, the status changes to "errored," which can be further specified using the \textit{hasErrorMessage} property.

Other important datatype properties for the execution include \textit{plannedStartTime} and \textit{plannedEndTime}, as well as \textit{realStartTime} and \textit{realEndTime}, which are added after completion. The actual performance of the execution may differ from the expected performance of the process, which is captured by the \textit{realPerformance} property connecting the execution to a performance with corresponding datatype properties.

Using the process execution model allows for both the inclusion of past, current and future events to the ontology. These then again contribute to the believes part of the BDI architecture, as well as constitute the intentions of the different agents in the \gls{mas}.
